Iterative Design of An Accessible Crypto Wallet for Blind Users

Crypto wallets are a key touch-point for cryptocurrency use. People use crypto wallets to make transactions, manage crypto assets, and interact with decentralized apps (dApps). However, as is often the case with emergent technologies, little attention has been paid to understanding and improving accessibility barriers in crypto wallet software. We present a series of user studies that explored how both blind and sighted individuals use MetaMask, one of the most popular non-custodial crypto wallets. We uncovered inter-related accessibility, learnability, and security issues with MetaMask. We also report on an iterative redesign of MetaMask to make it more accessible for blind users. This process involved multiple evaluations with 44 novice crypto wallet users, including 20 sighted users, 23 blind users, and one user with low vision. Our study results show notable improvements for accessibility after two rounds of design iterations. Based on the results, we discuss design implications for creating more accessible and secure crypto wallets for blind users.

==> txt/Finding_arxiv__metamask_.tex <==
% \zhixuan{the current qualitative findings are only exploratory, and based on notes taken during 10 user experiments on \textbf{MetaMask} with people without visual impairments.}

% Through this study, we aim to provide an overall understanding of the usability, education (learnability), security, and accessibility of crypto wallet. For each aspect, we will report on how users interact with MetaMask and our redesigned version, respectively, through the lens of both qualitative and quantitative evidence. 

% Qualitative evidence, specifically, observational notes taken by the first author during the experiments, and interview responses during the initial and exit interviews, is the main evidence for supporting our claims. 
% For usability, we further use task success rate and the SUS survey results to demonstrate how smoothly our participants were able to use the two wallets. 
% Educational effects are measured through two KQ surveys and the success rate of some tasks, with the assumption that users could answer the concept questions and conduct the tasks relating to the concepts (e.g., public key, private key, etc.) better if they are properly educated through the embedded education. 
% Wallet security can be inferred from some security-related tasks, e.g., if users are able to type the correct receiving address, and if they disclose their seed phrase for free token airdrops. 
% Accessibility of the wallets can also affect the success rate of multiple tasks. 

% According to the t-test, significantly more participants failed to find the transaction function (not properly labeled for screen reader users) and import their wallet (misconception about encryption) in our redesigned wallet. 
% No significant differences are found between the success rate of MetaMask and our redesigned wallet on other tasks. Thus we will mostly report on descriptive statistics for task success. The difference between the SUS survey responses for MetaMask and our redesigned wallet is also not significant.

\iffalse
% \subsection{MetaMask}

% \textbf{Overall Usability.}
% According to the SUS surveys, our participants rated 3.8 for metamask, showing a relatively high level of satisfaction.

% The complaints around usability mainly fell into the use of seed phrase. Our participants needed to store and confirm their seed phrase during the setup process, and use their seed phrase to import the existing wallet into a new device, both seen as cumbersome and time-consuming.

% MetaMask provides two ways of giving the seed phrase to users in the onboarding process, either downloading it into a txt file, or directly revealing the hidden 12-word string. Most participants chose to reveal the seed phrase and keep it manually, e.g., writing it down, taking a picture, or taking a screenshot on the computer, since this method was placed on the left side of screen, and thus was unintentionally prioritized. Several participants (e.g., M7) acknowledged ignoring the option of downloading their seed phrase on the right side, which they would have used. 

% In the next setup step, users are prompted to select and arrange the 12 seed phrase words into the correct order to confirm that they have stored it properly. M7 thought this way of confirmation was time-consuming, and preferred a more standardized way, e.g., typing, rather than selecting. The selecting process can be even harder for blind users. As in M18's case, when selecting the seed phrase words, for each word, she needed to check it in the original seed phrase, and go through the shuffled words to find the matching one --- this process was cumbersome using a screen reader. M15 also complained that this seed phrase confirmation process took them a lot of energy.
% % memory issues

% Since most of our participants kept the seed phrase in non-text forms, they had to manually type it during the importing process, which could lead to inefficiency and error. For example, M8 entered all capital letters for the seed phrase, and included some typos, which made him unable to import the wallet. M7 double-checked each word after typing it. Interestingly, though MetaMask provides a handy function with clear explanation ``you can paste your entire secret recovery phrase into any field,'' our participants still chose to type their seed phrase, probably due to their user habit.

% Some participants interestingly cared less about the usability aspect. For example, M8 thought ``security is the most important thing, and design is less important. It's okay if the
% import process is not smooth.'' However, usability designs can sometimes lead to security issues: MetaMask provides the option of skipping the seed phrase confirmation process (``remind me later'') during onboarding. Three of our participants skipped the process and did not bother to backup their seed phrase even though reminded by a popup during their wallet usage. They thought the onboarding process to be smooth and quick, but they were not able to import their wallet without the seed phrase.

% \textbf{Education/Learnability.}
% Except for M3 who was ``pretty familiar with wallet concepts due to exchange experience,'' all other participants thought there were way too many complicated concepts in MetaMask, which failed to educate novice users. M15 suspected that the ``complexity of the technical terms was intentional to get more money from people.'' Seed phrase, public key, private key, gas fee, cryptocurrency, password, and main vs. test networks were the concepts surrounded by the most confusion. While MetaMask use different media, such as text and video instructions, to provide users with necessary crypto and security knowledge, our participants perceived the effectiveness of the education differently based on their own user habits and levels of crypto knowledge.

% \textit{Video Instructions.} There is one video in MetaMask educating users on crypto and wallet basics. Most participants thought it was easy to understand and informative, though M10 thought it was too fast, and he had to pause and replay it. 

% Several participants skipped the video and attributed the choice to their user habits when using most apps. For example, M16 thought it unnecessary to watch the video to create an account. M17 identified himself as a hands-on person who usually tried out things and googled around, instead of following instructions. 

% For M14, a blind user, videos in apps were barely accessible in his experience: ``usually it's just visual and no sound.'' Yet another issue with MetaMask video is that it is only available in the onboarding process, and people cannot watch it later. M15, who skipped the video when setting up the wallet, said, ``I want to go back watching this video, but it's not available.''

% \textit{Text Instructions.}
% Text instructions, especially those beside the video, were ignored by several participants. M1 attributed to her overlooking the text to the existence of the video, and she suggested highlighting the text instructions. M10 also ignored the text for ``being more alerted by videos.''

% Blind users are more likely to unwillingly ignore the text, since the next button is placed on the left side right after the video, and text is placed on the right side. Many of them proceeded to the next page without noticing the text instructions, which contained important information such as the seed phrase security. M15 was the rare one who navigated things after the next button based on their personal experience and habit.

% Perceived uselessness of text instructions was also common among our participants. M17 perceived text instructions to be useless and skipped most of them in the onboarding process. After he failed the phishing task, he decided to follow the text instructions in the importing task. He thought he ``did better after reading through the text instructions.''

% \textit{Seed Phrase.} M4 directly expressed that she did not understand the meaning of seed phrase after the experiment. M1 did not realize the importance of the seed phrase even though she was informed of its importance by MetaMask, so she did not write it down after seeing it; only after she was prompted to confirm the seed phrase, she went back and wrote it down. M10 needed more emphasis on seed phrase in a more dedicated way. M16 thought the option of skipping seed phrase confirmation (``remind me later'') diluted the education on seed phrase, and he was no longer sure if the seed phrase was important.

% \textit{Public Key.} Nearly all our participants complained that the public key/wallet address was not intuitive enough, as in MetaMask, the string is simply put under ``Account 1.'' M11 said, ``The wallet address is just there, without any
% explanation, which makes me anxious.'' Beside, MetaMask only shows partial digits of the public address on its main page (e.g., 0xECe...6538), which made some participants (e.g., M13) think this was their full wallet address.

% Explanation can be as simple as ``this is my wallet address,'' as suggested by M10. Ignorance or misunderstanding of the public key can lead to security concerns: M5 gave the author her seed phrase, which is the only access to her wallet, when asked for her wallet address. She thought ``more instructions should be provided regarding public key,'' which was a term she had never come across before using the wallet.

% \textbf{Private Key.} When filling in the second KQ survey, M4 commented that she did not understand private key, since it never showed up during the experiment. 

% \textit{Gas Fee.} Our participants were curious what gas fee meant. M3 complaint that there was no education for gas fee. Some participants, like M6, suspected that gas fee might be a transaction fee equivalent, but none of them were sure about this concept. 

% No participant tried to adjust the gas fee during the transaction process. For example, M1 was confused about what percentage of the transaction amount she should pay as the gas fee. M10 was not aware that he could change the gas fee. M8 did not adjust the gas fee because ``it was a small amount.''

% \textit{Crypto.} According to our participants, MetaMask failed to provide any explanations on cryptocurrency or its relationship to fiat currency. M16 was not sure what Ethereum (or ETH as in MetaMask) means. M15 thought the real-time conversion rate between ETH and fiat currency, e.g., US dollars, should be given. M4 did not understand how to consume ETH in daily life settings, which made it less useful. She thought crypto wallets should play a role in teaching people how to use cryptos.

% \textit{Main vs. Test Networks.} We use the Ropsten test network and test ETH during the experiments. Some participants like M18 expressed that they did not understand what testnet meant. Upon importing his wallet, M9 nervously asked the author, ``where's my ETH?'' He was relieved only after the author helped him change to the Ropsten testnet and his Ropsten ETH balance was shown.  

% As we can see, MetaMask seems to be assuming that users are technically/cryptographically savvy, and does not provide much education on crypto concepts, such as seed phrase and gas gee, which are not at all understandable for novice users. What is worse, for the limited educational resources, our participants tended to skip them when using the wallet, which we will elaborate on below.

% \textbf{Security.}
% Our participants turn out very vulnerable to phishing attacks. Other perceived security risks associated with MetaMask include lack of education, lack of trust in chrome extensions, seed phrase security, not being centralized, receiving address accuracy, and accessibility-induced risks, which we will elaborate on hereby.

% \textit{Phishing Task.} Notably, 14 participants failed the phishing task out of all 18, for various reasons. Some, like M1, did not notice any warning for seed phrase security, so gave it to the phishing website without any hesitation. Some, like M14, did notice the warning but forgot about it after some time. M11 attributed to his recklessness to the persuasive power of the phishing website, and the mentality that it was only a study setting. Similarly, M7 also thought it was only a test or experiment: ``if it was actual money, I would have paid more caution.'' M8 disclosed his seed phrase for the free airdrops (financial incentive) even when realizing the danger. M15 was confused about the phishing website after ``already being confused about the crypto concepts.''
% M18 - Phishing: not a good idea; confused:
% seed phrase, not secret recovery phrase  

% \textbf{Security Perceptions and Risks.}
% MetaMask has been recognized as a safe crypto wallet by most of our participants. For example, M18 attributed her positive perception about the wallet security to the protection provided by password and seed phrase. M9 thought the wallet was simple (good usability) but not so simple (seed phrase protection), thus was safe. 

% \textit{Lack of Education.}
% Security perception is closely related to the information and education resources provided by the wallet, which can help users make more informed decisions and feel more safe. M1 said she was provided too little information by the wallet to feel safe, and she needed to know more about cryptocurrencies, who controls blockchains.

% \textit{Distrust in Chrome Extensions.}
% Some participants did not trust chrome extensions due to a lack of familiarity (M6) and frequently reported personal information leakage through chrome extensions (M7). M5 explained, ``I trust the wallet less than PayPal because it's not always there in a link (e.g., https://www.paypal.com/). I need to install the chrome extension into my browser.'' 

% \textit{Seed Phrase Is Not Safe.}
% Seed phrase itself is seen as a vulnerable crypto management mechanism by some. M9 chose to write his seed phrase down instead of copying and pasting it to the computer, which he thought was unsafe. M6 had a similar concern: he thought it was difficult to remember the seed phrase, and he had to store it in different devices, which made it more likely to be exposed to attackers. M8 commented that the wallet itself was secure, and its security depended on ``how carefully you take care of the seed phrase.'' However, none of our participants was able to think of a way to prevent seed phrase loss and seed phrase theft at the same time.

% M14 - (Onboarding) Download the seed
% phrase and remind me later (good)

% \textit{A Centralized Mentality.}
% A country-specific security perception was found in participants from China or those who had a Chinese background. Many of them felt unsafe since the wallet was decentralized. M5 said she would feel safer if the wallet asked for her ID or phone number, because in that way, it would be able to trace her money back. M6 showed little trust in crypto wallets, since they were not linked to centralized banks. M10 said he would have more trust in the wallet if it is backed by United Nations or other centralized organizations. He acknowledged this to be a paradoxical mindset where he valued decentralization and anonymization, and the perceived security provided by centralization at the same time. Such a mentality might be attributed to the fact that Chinese people have been used to centralized apps, and they had to provide their ID and phone number in order to use any app \cite{exchange}. 

% However, this centralized mentality may change after people are exposed to the principles of cryptocurrency and crypto wallets. For example, before the experiment, M9 did not want to transfer money into crypto wallets which were not ``really famous or run by well-regulated companies.'' He was concerned that he did not know where MetaMask was based, and that his wallet address and seed phrase would disappear if MetaMask went bankrupt. However, he trusted wallets more than centralized exchanges after we explained the decentralized and anonymous nature of blockchains.

% \textit{Sending to the Wrong Address.}
% M9 who manually typed the receiving address during the transaction task expressed the fear of typing it wrong. Those who copied and pasted the author's address were also not sure. For example, M7 said to the author ``this looks like you,'' after entering the receiving address. Several participants expressed their worry of sending ETH to the wrong address, and attributed the concern to the lack of an address confirmation page in MetaMask.
% Several mentioned that crypto wallets should be simple but not so simple to be safe, otherwise it was easier for attacks to happen (M9). M7 explained that the UI of MetaMask was so intuitive, and she easily skipped the security warnings because of that.

% \textit{Accessibility and Security.}
% Blind users expressed their concern about MetaMask for its accessibility issues such as unlabeled buttons, which could lead to security vulnerabilities. M11 explained how accessibility could impact security: ``with some of the functionalities unclear to me as a screen reader user, it
% raises some trust concerns in that I'm afraid to set off some unknown function that could negatively impact my account, for example, accidentally clicking the wrong button and
% making my account number available to the clipboard without awareness. That could be a real problem if I were using this wallet on public channels.'' The accessibility challenges will be addressed in later sections.

% \textbf{Accessibility.}
% According to some participants, ``accessibility of cryptocurrency itself is good. It's digital; blind people have difficulty telling the face value of paper money.'' (M11) However, except for M16 who thought accessibility issues of MetaMask were manageable, all other blind participants were more or less discouraged by accessibility issues, including incompatibility with screen readers, lack of sound notifications, and the cumbersome process dealing with the seed phrase. Accessibility issues can even lead to security concerns.

% \textit{Incompatiblility with Screen Readers.} According to M13 and many other participants, buttons in MetaMask were not properly labeled to be readable by screen readers\footnote{Our participants mostly use JAWS, NVDA, and Voiceover (only available in Mac systems).}, which makes wallet usage awkward for blind users. 

% In the onboarding process, M11 failed to set up his password promptly since the password rule (``8 character min'') was not readable by his screen reader. He also could not reveal the hidden seed phrase in the onboarding process, since the ``click here to reveal secret words'' button was hard to find and click on; thus he could not go to the next page without the help of the author. 

% During the transaction process, the place to enter transaction amount, as well as the button to change the amount between ETH and US dollar, are also not labeled (M11), making the transaction a rather time-consuming process for the blind users. M13 did not realize she could enter a number for the transaction amount. For some checkboxes, screen readers think they are unchecked even after the users have checked them (M18).

% M14 - Quite accessible except some
% unlabeled buttons, just need to click
% M16 - Important buttons unlabeled
% M18 - Headings: want it easier to jump around
% from place to place
% M18 - Unlabeled button

% \textit{No Sound Notifications.}
% Sound notifications are not often provided in MetaMask after an operation is conducted, e.g., copying the public key, and the transaction being confirmed on the network.

% On the wallet main page, the public key is provided under ``Account 1.'' After one hovers over this clickable button with her mouse, a text popup would show up saying ``Copy to clipboard.'' However, if a blind user navigates to this button with a keyboard, the text will not be verbally announced. Many of our blind participants like M13 did not know how to copy the wallet address until being told by the author to press the Enter key on the unlabeled button. Also, there was no announcing after the address was copied (M11).

% % M11 - No error message if transaction failed
% Transactions take time to be confirmed on the Ethereum network. A pending sign is shown during the waiting period, and disappears after the transaction is confirmed. It is relatively easier for sighted users to notice this visual update, for blind users, however, it is less noticeable (M13).
%  % - Tell completed transaction by pending
% Many of them alternatively inferred the transaction statues by checking the wallet balance. For example, before the transaction, M14 had 1.1 ETH, and after the transaction was confirmed, he was left with 0.1 ETH. M16 thought this evidence was not clear enough and was hard to identify.

% \textit{Seed Phrase.}
% As in M18's case, when selecting the seed phrase words, for each word, she needed to check it in the original seed phrase, and go through the shuffled words to find the matching one. This process was cumbersome with a screen reader. M15 also complained that this seed phrase confirmation process took they a lot of energy. 
% As reported before, blind users have to devote much time and energy to confirming their seed phrase word by word during the onboarding process. Some of them, like M11 and M13, did not want to go back and forth to confirm the seed phrase, and chose to use the ``remind me later'' option to skip this process of saving and confirming the seed phrase.
% % M13 - “Remind me later”: next button is
% % grayed; after clicking, no notifications
% M11 backed up his seed phrase after being reminded to do so when using the wallet, and M13, on the other hand, ignored the reminder and ended up being unable to import her wallet since she did not have the seed phrase.

% \textit{Accessibility and Security.}
% The accessibility issues mentioned above have exposed our blind participants to some security risks. M13 pessimistically commented that ``accessibility makes it hard to think
% about security.'' In the education section, we have reported that blind users tend to ignore important information in text after the Next button (M11, M13).
% M13 - Next button put after video, and
% before text: missing important information
% Besides, since there was no announcing after the receiving address was pasted during the transaction, M14 was concerned about typing the wrong address. A better design could have been to announce the entered receiving address.

==> txt/Finding_arxiv__v1_.tex <==
\subsection{Redesigned Wallet (V1)}

\textbf{Overall Usability}
% (\sout{qualitative}, \sout{task success rate}, \sout{SUS survey)}
Our participants rated 3.8 for metamask and similarly 3.6 for our wallet out of 5 (1 means totally negative about usability, 3 means neutral, and 5 means totally positive about usability), slightly above neutral.

Our wallet prioritizes the option of downloading the seed phrase during the onboarding process by putting it on the left side and seed phrase revealing on the right side of the same screen. Out of security concern, we prompt users to use a 6-digit pin to encrypt their seed phrase before it is downloaded to their local computer. Without the pin, attackers will not be able to decrypt and see the seed phrase. During the evaluation, 15 out of 18 participants used this option to keep their seed phrase, showing the effectiveness of the nudging. W9, who was among the rare ones writing down their seed phrase, noted confirming seed phrase in their original order was hard. When importing her wallet, she had to manually type the seed phrase, and did not contain space between the words at first, which cost her quite some time to import the wallet.

This usability/security design, however, has caused some new usability issues. After introducing the new concept of pin, some participants, like W1, were confused regarding how password, pin and seed phrase should be used in different circumstances. While we, as security researchers, take the concepts of encryption/decryption for granted, for our participants, they were confusing. W2, and W10 alike,  expressed her confusion around seed phrase encryption throughout the experiment.

Another design flaw is that in the importing process, we forget to consistently prioritize the uploading option over manually entering the seed phrase. Nine of our participants failed to finish the import task, because they tried to copy and paste their encrypted seed phrase into the left-side blank, which only accepted seed phrase in the form of 12 words. W7 focused on the left side (manually entering) during the importing process, and W11, a blind user, said she had wanted to import seed phrase with the downloaded file, but failed to find the uploading option since it was on the right. As a result, only 8 participants were able to successfully import their wallet, while 14 participants were able to do so in MetaMask (p<0.05). As we can see, the placement/prioritization of functions on a page can make a huge difference to user behavior, and it is more so for screen reader users, who have more difficulty navigating around the page. The importing process also showed the ignorance of our participants regarding encryption, which we did not take into account when designing the encryption/decryption feature. However, given more time, the participants would be able to find and use the option of decrypting and uploading the encrypted/downloaded seed phrase --- the seed phrase will not be lost.
% W12 - Upload file option should be on the left
% W14 - Preferred uploading the seed phrase
% file
% W15 - Prioritize the upload option

Language barrier was indicated by W7 from China, who preferred to use a Chinese version of our wallet. For her, the most unusable part of the wallet was that she had to understand the English before she could use the functions.

\textbf{Education/Learnability}
In addition to the video provided by MetaMask, we added three videos (What are cryptocurrencies? What is a blockchain? What are wallet \& exchanges?) in a dedicated ``basics'' page at the very beginning of the onboarding process, one video for explaining the importance of password when users are prompted to create their device-specific password, and one video for explaining gas fee in the transaction page. We also implemented a chatbot in the wallet where users can ask crypto/wallet related questions. 

Our designs were shown effective in educating novice user on crypto concepts. In the first KQ survey before the tasks, participants for MetaMask were able to answer 3.4 out of the 7 questions correctly on average, and participants for our wallet were able to answer 3.7 of them correctly. In the second KQ survey after the tasks, participants for MetaMask were able to answer 3.7 of the questions correctly, showing an improvement of only 0.3, whereas the average score of the participants for our wallet jumped to 4.4, showing an improvement of 0.7. After using our wallet, 16 participants understood public key, increasing from 6 prior to the use; 2 participants understood the factors influencing gas fee, compared to 0 for MetaMask users.

Below we reflect on our designs and the educational effects of these designs.

\textit{Video Instructions.} Regarding videos, several participants skipped them for similar reasons as in the MetaMask experiments: user habit (e.g., W1), perceived uselessness (e.g., W10, ``skip everything but can still get it set up''), preferring text over video (e.g., W15, ``I'm a text person''). However, more participants perceived the videos to be useful, and they were willing to watch the minutes-long videos. W3 thought the videos on the first page caught her eyes. W5 suggested making the videos mandatory, which could correct the ``bad user habit'' of skipping instructions. W3 further suggested embedding a video to educate users on crypto-related laws. One drawback of the videos was mentioned by W18, who thought the cryptocurrency video was jargon heavy. Since we borrowed the videos from online sources, e.g., YouTube, we were not able to create jargon-free videos for novice users, which we see as a future work.

\textit{Chatbot.} None of our participants used the chatbot, mostly for the ``skipping everything mentality'' (W5). W1 further pointed out the poor performance of chatbots: ``from my experience, chatbots aren't very efficient in other websites. They can't concisely answer questions.''

\textit{Seed Phrase.} Our option of encrypting and downloading the seed phrase might negatively affect users' understanding of this concept, since they are never exposed to the 12 words, but instead a ``random string,'' as complained by W1. W16 was confused that he was not shown the original seed phrase, yet was asked to enter the words in the importing process (``Secret Recovery Phrases contain 12, 15, 18, 21, or 24 words'').

\textit{Gas Fee.} Though we added a video to explain gas fee, as well as a gas fee glider to adjust it, still none of our participants tried to adjust the gas fee, even if it was perceived as ``a lot'' (W6). W1 thought gas fee was something like tax and unavoidable, and he did not know he could adjust it. W5 thought the gas fee was fixed. W10 did not notice gas fee and asked the author after transaction: ``I should be left with 6 ETH, but it's only 5.99999.''

Toward better educating novice users on crypto concepts, W1 suggested providing more instructions for new users; W2 suggested a dedicated section for explaining crypto concepts; W8 suggested a zone for new users which only had basic functions. 

\textbf{Security}
The participants had similar security perceptions in our wallet to MetaMask. For example, they did not think they were ``knowledgeable enough to feel safe.'' (W1) Standalone apps were preferred over Chrome extensions: ``I'm not sure if I'm on the extension or some website pretending to be the extension.'' (W17) 

\textit{Phishing Task.} Despite providing more video and text instructions regarding seed phrase security in the wallet, we did not see an improvement in the success rate of the phishing task. Only 3 participants passed the phishing test without giving their seed phrase to the phishing website. People's reasons for disclosing their seed phrase are not much different from those found in the MetaMask experiments; additionally, W5 and W12 thought ``the phishing website was linked with the wallet.'' W9 suggested more warnings for beginners, for example, ``it's a very keyword, just like the password of your debit card.'' 

Interestingly, since most of the participants (15 out of 18) did not have access to the original seed phrase, but instead the encrypted version in the downloaded txt file, they submitted the encrypted seed phrase to the phishing website to claim the airdrop --- our encryption design unintentionally prevents users from the risk/loss from phishing attacks. Our participants, like W5, did ``feel safer for the pin-enabled encryption of the seed phrase.''

Below we elaborate on other security improvements afforded by our designs.

\textit{Making Seed Phrase Saving Compulsory.}
While we removed the ``remind me later'' option during the onboarding process, the participants had to save and confirm their seed phrase, and thus all of them had access to their seed phrase throughout the experiment; as a comparison, three  participants for MetaMask used this option during setup and failed the importing task later. 

\textit{Double-checking Receiving Address.}
The added feature of requiring users to check the receiving address by re-entering the last 4 digits has also helped. For example, in this step, W2 noticed the wrong receiving address she initially entered: ``it nudged me to check the address. I liked this feature.'' Only 1 participant sent the ETH to the wrong address, compared to 4 in the MetaMask group. 

% W6 - Phishing: thought was just entering
% account and password
% W7 - Didn’t notice seed phrase warning
% W9 - Noticed the seed phrase warning but
% didn’t remember it
% W10 - Remember the seed phrase warning,
% but don’t know it’s a scam website
% W12 - Thought the phishing website was
% linked to the wallet; free tokens
% W18 - Didn’t remember the seed phrase
% security


\textbf{Accessibility}
While we labeled the unlabeled buttons in MetaMask, several designs have introduced new accessibility issues, mainly because of the incompatibility of popups with screen readers (W18). The seed phrase confirmation popup asking users to upload their downloaded, encrypted seed phrase during the onboarding process was not readable by NVDA (W11). The transaction confirmation popup page (W15) and chatbot popup (W12) brought similar accessibility issues. W13 did not know how to quit the chatbot, since his screen reader kept focusing on the popup instead of the main page.
% W11 - Wallet address not recognized by NVDA
%W12 speculated that screen readers always had difficulty reading things on the second level.

% W12 - Wallet address not recognizable
% W12 - Cannot click on send button
% W13 - Chatbot: focus not always on the
% message enter space
% W13 - Three videos: all “play button”
% W13 - Unlabeled buttons
% W14 - Send button not labeled
% W15 - Send button not recognizable by MacVoiceover

% W17 - Copy button for the wallet address
% W17 - Popup accessibility: focus
% W18 - Popup not accessible
% W18 - Buttons not labeled, only text provided

% \textbf{No Sound Notifications.}
% W8 - Checked activity; maybe it’s finished;
% didn’t show most recent transaction; inferred
% by balance
% W18 - Didn’t announce copying wallet address

% \textbf{Accessibility and Security.}
% W16 - Prefer next button at the bottom of
% the page
\fi
